Contact angle of sessile drops in Lennard-Jones systems

Molecular dynamics simulation is used for studying the contact angle of nanoscale sessile drops on a planar solid wall in a system interacting via the truncated and shifted Lennard-Jones potential. The entire range between total wetting and dewetting is investigated by varying the solid--fluid dispersive interaction energy. The temperature is varied between the triple point and the critical temperature. A correlation is obtained for the contact angle in dependence of the temperature and the dispersive interaction energy. Size effects are studied by varying the number of fluid particles at otherwise constant conditions, using up to 150 000 particles. For particle numbers below 10 000, a decrease of the contact angle is found. This is attributed to a dependence of the solid-liquid surface tension on the droplet size. A convergence to a constant contact angle is observed for larger system sizes. The influence of the wall model is studied by varying the density of the wall. The effective solid-fluid dispersive interaction energy at a contact angle of 90 degrees is found to be independent of temperature and to decrease linearly with the solid density. A correlation is developed which describes the contact angle as a function of the dispersive interaction, the temperature and the solid density. The density profile of the sessile drop and the surrounding vapor phase is described by a correlation combining a sigmoidal function and an oscillation term.

==> TOC.tex <==
% TOC
\section{Graphical TOC Entry}

\begin{figure}[htb]
\includegraphics[height = 8.333cm]{TOC.png}
\end{figure}


==> figureFile.tex <==
\section{Figures}


\begin{figure}[htb]
 \includegraphics[width = 8.333cm]{SimulationSnapshot.eps}
 \caption{Simulation snapshots taken with VMD\cite{Hump96} at a temperature of $T = 0.8 ~\epsilon_f / k$. The reduced solid--fluid interaction energy
	  is $\zeta = 0.25$ (left) and $\zeta = 0.65$ (right), resulting in different contact angles.}
 \label{fig:Snapshots}
\end{figure}
\newpage

% density profile
\begin{figure}[htb]
\includegraphics[height = 8.333cm]{Sim_N15t_T08_xi0065.eps}
\includegraphics[height = 8.333cm]{Sim_N15t_T09_xi0025.eps}
\caption{Density profiles of liquid droplets. 
	 The color indicates the density in units of $\sigma_f^{-3}$.
	 The white circle is fitted to the interface at the positions with $\rho = (\rho' + \rho'')/2$ 
	 and employed to determine the contact angle by extrapolating to $y = 0$.
	 Left: The reduced solid--fluid interaction energy is $\zeta = 0.65$ 
	 and the temperature $T = 0.8~\epsilon_f/ k$. 
	 An adsorbed fluid phase can be observed next to the droplet.
	 Right: Density profile of a droplet under conditions of total dewetting. 
	 The simulation parameters are $\zeta = 0.25$ and $T = 0.9 ~\epsilon_f/ k$.}
\label{fig:SampledDensProfile2D}
\end{figure}


%size effects results
\begin{figure}[htb]
  \includegraphics[width = 8.333cm]{SizeEffects.eps}
 \caption{Impact of the number of fluid particles $N$ in the simulation box on the contact angle $\theta$ at $T = 0.8~\epsilon_f/k$ and 
	  reduced solid--fluid interaction energies $\zeta$ of 
	  0.35 ($\triangle$),
	  0.5 ($\Diamond$) and
	  0.65 ($\circ$).
	  The dotted lines correspond to the average of the results for the three largest particle numbers $N$.}
 \label{fig:SizeEff}
\end{figure}


% axial density profile
\begin{figure}[htb]
\includegraphics[width = 8.333cm]{FittedDensityProfile_N15t_T08_xi0065.eps}
\includegraphics[width = 8.333cm]{Sim_rhoAxial_N15t_T08_xi0065.eps}
\caption{Left: Correlation, cf. Eq.~\eqref{eq:densityCorrlationFnk}, of the density profile of a liquid drop adjusted to the data 
	 shown in \ref{fig:SampledDensProfile2D}, i.e. for a sessile drop at $\zeta = 0.65$ 
	 and $T = 0.8~\epsilon_f/ k$. 
	 Left: Two dimensional profile as obtained by the Eq. \eqref{eq:densityCorrlationFnk}.
	 The color indicates the density in units of $\sigma_f^{-3}$.
	 Right: Simulation results~($\circ$) and correlation ~(--), cf Eq.~\eqref{eq:densityCorrlationFnk},  for the density profile along
	 the axis of symmetry of the droplet ($R=0$) over distance from the wall.}
\label{fig:SampledDensProfile1D}
\end{figure}



% empirical correlation, var xi
\begin{figure}[htb]
 \includegraphics[width = 8.333cm]{cos_Korrelation_xi_T_const.eps}
 \caption{Simulation results (symbols) and correlation (lines), cf. Eq.~\eqref{eq:eqCorrelationCA}, for the contact angle 
 as a function of the reduced solid--fluid interaction energy at temperatures of $T = $ 
  $0.7$ ($\circ$, \hdashrule[0.5ex][x]{1.0cm}{0.8pt}{}),
  $0.8$ ($\triangle$, \hdashrule[0.5ex][x]{1.2cm}{0.8pt}{2.5mm 3pt 0.5mm 3pt}),
  $0.9$ ($\square$, \hdashrule[0.5ex][x]{1.3cm}{0.8pt}{5mm 3pt}),
  $0.95$ ($\triangledown$, \hdashrule[0.5ex][x]{1.2cm}{0.8pt}{2pt}) and
  $1.0~\epsilon_f/k$ ($\Diamond$, \hdashrule[0.5ex][x]{1.2cm}{0.8pt}{2.5mm 3pt 2.5mm 3pt 2.5mm 3pt}).
  The wall density is $\rho_s = 1.07~\sigma_f^{-3}$, i.e. $\sigma_s = \sigma_f$.}
  %Correlation~\eqref{eq:eqCorrelationCA}~(--).}
  \label{fig:CAcorrelation1varxi}
\end{figure}


% empirical correlation, var T
\begin{figure}[htb]
  \includegraphics[width = 8.333cm]{cos_Korrelation_T_xi_const.eps}
 \caption{Simulation results (symbols) and correlation (lines), cf. Eq.~\eqref{eq:eqCorrelationCA}, for the contact angle 
 as a function of temperature at values of the solid--fluid interaction energy $\zeta$ of
 $0.25$ ($\circ$),
 $0.3$ ($\square$),
 $0.35$ ($\triangle$), 
 $0.4$ ($\triangledown$),
 $0.5$ ($\Diamond$),
 $0.6$ ($\hexagon$),
 $0.65$ (\FiveStarOpen) and 
 $0.75$ ($\RIGHTcircle$).
 The wall density is $\rho_s = 1.07~\sigma_f^{-3}$, i.e. $\sigma_s = \sigma_f$.}.
 \label{fig:CAcorrelation1varT}
\end{figure}



\begin{figure}[htb]
  \includegraphics[width = 8.333cm]{wettingTemperature.eps}
 \caption{Transition temperature $T_w$ towards total wetting ($\theta = 0^\circ$) or dewetting ($\theta = 180^\circ$) normalized 
 by the critical temperature $T_c$ as obtained from Eq.~\eqref{eq:eqCorrelationCA}. }
 \label{fig:wettingTemperature}
\end{figure}




% average potential well depth over solid density
\begin{figure}[htb]
\includegraphics[width = 8.333cm]{W0_vs_rho_s_linear_InclNijmeijerLongRange}
\includegraphics[width = 8.333cm]{alphaBar_vs_rho_s_linear_InclNijmeijerLongRange.eps}
\caption{ Left: Value of $W_0$, corresponding to the average minimum potential that yields $\theta = 90^\circ$, for wall models of different density.
	  Right: Gradient $\bar{\alpha}$ of the contact angle cosine over the solid density.
	  This work: $\rho_s = 1.07 \sigma_f^{-3}$ ($\blacktriangle$), 
		     $\rho_s = 2.10 \sigma_f^{-3}$ ($\blacksquare$), 
		     $\rho_s = 4.02 \sigma_f^{-3}$ ($\Diamondblack$). 
	 Ingebrigtsen and Toxvaerd \cite{Ingebrigtsen2007} ($\Circle$);
	 Grzelak et al. \cite{Grzelak2010a}, bcc~(100) lattice ($\triangledown$);
	 Tang and Harris \cite{Tang1995} ($\square$);
	 Nijmeijer et al. \cite{Nijmeijer1990} ($\triangle$);
	 Nijmeijer et al. \cite{Nijmeijer1992} combined model ($\Diamond$);
%	 Horsch et al.~\cite{Horsch2010}~($\RIGHTcircle$).
	 The lines represent the fit obtained using from the present simulation data using Eqs.~\eqref{eq:W0Linear} and \eqref{eq:alphaBarOverRhoWall}.
	 The parameters are $\eta_1 = 3.6$, $\eta_2 = 1.1$, $\eta_3 = -0.04$, and $\eta_4 = 0.38$.}
\label{fig:W0OverRhoS}
\end{figure}






% cos_theta predicted
\begin{figure}[htb]
 \includegraphics[width = 0.5\textwidth]{figures/prediction_cosThetaInclNijmeijerLongRange.eps}
 \caption{Contact angle cosine over the absolute magnitude $W$ of the average minimum potential.  
  The lines represent Eq.~\eqref{eq:CAPredicted} with the parameters $\eta_1 = 3.6$, $\eta_2 = 1.1$, $\eta_3 = -0.04$, and $\eta_4 = 0.38$.
  The symbols are the simulation results at different temperatures $T$. 
  This work at a temperature of $0.8 \epsilon_f / k$:
  $\rho_s = 1.07 \sigma_f^{-3}$ ($\blacktriangle$), 
  $\rho_s = 2.10 \sigma_f^{-3}$ ($\blacksquare$), 
  $\rho_s = 4.02 \sigma_f^{-3}$ ($\Diamondblack$).
  Ingebrigtsen and Toxvaerd \cite{Ingebrigtsen2007}, $0.75 \epsilon_f / k$, ($\Circle$);
  Grzelak et al. \cite{Grzelak2010a}, bcc~(100) lattice, $0.70 \epsilon_f / k$, ($\triangledown$);
  Tang and Harris \cite{Tang1995}, $0.90 \epsilon_f / k$,($\square$);
  Nijmeijer et al. \cite{Nijmeijer1990}, $0.90 \epsilon_f / k$, ($\triangle$);
  Nijmeijer et al. \cite{Nijmeijer1992} combined model ($\Diamond$).
  The simulation results and the corresponding lines representing Eq.~\eqref{eq:CAPredicted} are linked by the colors.}
 \label{fig:CAPredicted}
\end{figure}


==> tableFile.tex <==
\section{Tables}


% Model details of different simulations of contact angles
\begin{table}[hb]
\caption{LJ model systems used for studies on wetting. The solid--fluid potential of 
Ingebrigtsen  and Toxvaerd \cite{Ingebrigtsen2007} is a continuous LJ~9--3 model, all other potentials are particulate LJ~12--6 models.
The values of $W/\zeta$ were obtained from the literature sources (see text). 
The parameters $W_0$ and $\bar{\alpha}$ of a correlation of the literature data based on Eq. \eqref{eq:eqCorrelationCAReduced} are given.}
\begin{tabular}{ | c | c | c |c | c | c | c |}
\hline 
source 					& $\rho_s$/  		& $r_{c,sf}$/  		& $T$ /			&$W $ / 	& $W_0$ /	& $\bar{\alpha}$\\
~					& $\sigma_f^{-3}$ 	& $\sigma_f$		& $\epsilon_f / k$ 	&$\zeta k T_c$	& $k T_c$	& 		\\	
\hline
Ingebrigtsen    			& 0.60 			& $\infty$ 		& $0.75$		&$1.32$		& $1.37$	& $0.356$	\\
and Toxvaerd \cite{Ingebrigtsen2007}	& ~			& ~			& ~			&~		& ~		& ~		\\
\hline
Grzelak et al. \cite{Grzelak2010a} 	& 0.58			& $5.00$		& $0.70$		&$3.00$		& $1.38$	& $0.376$ 	\\
bcc(100) lattice			&~ 			&~ 			&~ 			& ~		&~ 		&~ 		\\	
\hline
Tang and Harris \cite{Tang1995}		& 0.62			& $ 2.75$		& $0.90$		&$2.62$		& $1.45$	& $0.323$	\\
\hline
Nijmeijer et al. \cite{Nijmeijer1990}	&1.78			& $2.21$		&$0.90$			&$3.61$		& $1.58$	& $0.371$ 	\\
\hline
Nijmeijer et al. \cite{Nijmeijer1992}	&1.78			& $2.35$		&$0.90$			&$4.03$		& $1.22$	& $0.338$ 	\\
combined model				& ~			& ~			& ~			& ~		& ~		& ~		\\
\hline					
%Horsch et al. \cite{Horsch2010}		& 5.88			& $2.50$ 		& $0.82$		&$17.29$	& $2.06$	& $0.246$	\\
%\hline
%Bucior et al. \cite{Bucior2009} 	&  --			& $2^{1/6}$		& $0.94$		& ~ 		& $[3.8,3.3]$ 	&--		\\
%\hline
~					& 1.07			& 2.50			& $0.80$		&$3.08$		& $1.58$ 	& $0.335$	\\
\cline{2-7}
this work				& 2.10			& 2.50			& $0.80$		&$4.83$		& $1.82$ 	& $0.288$	\\
\cline{2-7}
~					& 4.02			& 2.5			& $0.80$		&$8.07$		& $2.67$ 	& $0.215$	\\
\hline
\end{tabular}
\label{tab:ComparativeModelDetails}
\end{table}
\newpage
